Representation Matters: Assessing the Importance of Subgroup Allocations in Training Data

Collecting more diverse and representative training data is often touted as a remedy for the disparate performance of machine learning predictors across subpopulations. However, a precise framework for understanding how dataset properties like diversity affect learning outcomes is largely lacking. By casting data collection as part of the learning process, we demonstrate that diverse representation in training data is key not only to increasing subgroup performances, but also to achieving population level objectives. Our analysis and experiments describe how dataset compositions influence performance and provide constructive results for using trends in existing data, alongside domain knowledge, to help guide intentional, objective-aware dataset design.

==> intro_old.tex <==
\section{Introduction and Goals (old)}
A common hypothesis for why some machine learning models suffer low accuracy on subgroups of instances (e.g. gender classifiers perform worse for darker skinned females \citep{buolamwini2018gender}), is that there is insufficient representation of these subgroups in the training data sets. Therefore, a straightforward remedy would be to collect more data for these subgroups, and retrain the model (in fact, this is what Microsoft did in response to the gender shades study, according to their \href{https://blogs.microsoft.com/ai/gender-skin-tone-facial-recognition-improvement/}\todo{also cite https://dam-prod.media.mit.edu/x/2019/01/24/AIES-19\_paper\_223.pdf}{\textcolor{blue}{\underline{blog post}}}, and ImageNet has been updated to re-balance the presence of different images involving humans \citep{yang2020towards}). 

In this work, we study the effect of subgroup representation (what we will call \emph{heterogeneity} or  \emph{diversity} following \cite{mitchell2020diversity}) in machine learning datasets, across many prediction domains and classifier forms. We aim to make firm the understanding that data representation directly improves subgroup accuracy, and to go beyond this intuitive claim to generalizable insights as well as an understanding of the nuances present for different prediction domains and data set characteristics. 
%
\textbf{Our main goal is to  investigate the effect of subgroup representation in training data sets on the accuracy of a resulting machine learning model, evaluated across subgroups}. The major components of this study are designed to assess:
\begin{itemize}
    \item With standard training procedures that do not account for unequal subgroup training set representations, we model the empirical performance for subgroups, as a function of the percent of the training data set belonging to that subgroup. Further, \emph{can alternative schemes designed to handle small subgroup representations 
    %(up-weighting, group-distributionally robust optimization) 
    mitigate degradation due to smaller subset sizes, and when might they actually hurt performance?}
    \item Under a model of group accuracy as a function of the training set representations, understand the `optimal' training set allocation strategy to maximize population accuracy.
    In particular, \emph{does maximizing population accuracy coincide with under-sampling minority instances?}
    \item Investigate the signals in existing data sets that can guide training set allocations for future dataset collections. In particular, \emph{when and how can we use small datasets as ``pilot samples'' to inform group allocations in a subsequent data set collection?}
    % \item Connections to recent phenomena in machine learning; in particular, for data sets and contexts where it is a appropriate, we look at subgroup representations as a way to think about distribution shift.
\end{itemize} 
%
In this work, we study \textbf{representation} as the numerical inclusion of a predefined subset of groups in a data set. 
%
Numerical representation is just one facet of representation bias \cite{suresh2019framework}, which itself only on component of intertwined and more nuanced questions of what it means to achieve more diverse, inclusive, and truly representative sets, as well as to achieve equitable or fair outcomes for all \citep{mitchell2020diversity,buolamwini2018gender}. \todo{maybe switch this cite to Deb's}
%
Our results will highlight the importance of group representation even for population-level objective functions, suggesting that diverse training set representation is crucial for achieving accuracy, as well as fairness and equity. 


In reality, designing the data collection process to achieve desirable training sets will necessitate critical and diverse perspectives on what data collection and representation entails, both from a centralized data-collector perspective, and from the perspective of individuals about whom data is collected \citep{denton2020bringing}.
We expand upon this point in \cref{sec:limitations_future_work}, and until then focus on this notion of binary representation as a mathematically abstractable component of this much larger picture.
%
Our findings are summarized in following: \todo{ revisit this list of contributions after scaffolding the full outline}
\begin{enumerate}
    \item When the loss function (to be minimized) is separable, and  group-specific losses follow an inverse power law relationship with respect to their representation in the training set, and when observation noise is consistent across groups or higher for the minority group, the optimal allocation strategy to minimize \emph{population} level loss \emph{over-represents} minority groups in a training sample of fixed total size.
    \item{Using empirical data from diverse domains, across combinations of imaging and feature-based datasets, we demonstrate the importance of heterogenity in training data for \emph{population level}, as well as \emph{group level} accuracies.}
    \begin{enumerate}
        \item{We find empirically that up-weighting schemes such as importance sampling and GDRO do little to mitigate low subgroup accuracies when training set representation is low, compared to the relatively larger effect of changing the training set composition.}

    \end{enumerate}
    \item{We propose and evaluate different procedures for using small data sets to inform future sampling processes. 
    \begin{enumerate}
    \item{The return to additional data from other groups can be modeled in many settings, though some empirical results show more nuanced results, suggesting these results may be more context-dependent, and exposing avenues for important future work.}
    \end{enumerate}}
\end{enumerate}
